Gender Differences in Motivated Reasoning

Men and women systematically differ in their beliefs about their performance relative to others; in particular, men tend to be more overconfident. This paper provides support for one explanation for gender differences in overconfidence, performance-motivated reasoning, in which people distort how they process new information in ways that make them believe they outperformed others. Using a large online experiment, I find that male subjects distort information processing in ways that favor their performance, while female subjects do not systematically distort information processing in either direction. These statistically-significant gender differences in performance-motivated reasoning mimic gender differences in overconfidence; beliefs of male subjects are systematically overconfident, while beliefs of female subjects are well-calibrated on average. The experiment also includes political questions, and finds that politically-motivated reasoning is similar for both men and women. These results suggest that, while men and women are both susceptible to motivated reasoning in general, men find it particularly attractive to believe that they outperformed others.

==> fne_unskewed_priors.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                                   &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Unskewed                           &   -0.010&   -0.011&   -0.011&    0.007\\
                                   &  (0.009)&  (0.009)&  (0.010)&  (0.013)\\
Pro-Party News                     &    0.083&    0.037&    0.028&    0.075\\
                                   &  (0.007)&  (0.014)&  (0.008)&  (0.008)\\
Unskewed x Pro-Party               &    0.016&    0.015&    0.018&    0.007\\
                                   &  (0.012)&  (0.019)&  (0.013)&  (0.013)\\
Partisanship x Pro-Party           &         &    0.097&         &         \\
                                   &         &  (0.024)&         &         \\
Unskewed x Partisanship x Pro-Party&         &    0.006&         &         \\
                                   &         &  (0.032)&         &         \\
Anti-Party News                    &         &         &   -0.052&         \\
                                   &         &         &  (0.008)&         \\
Unskewed x Anti-Party              &         &         &    0.001&         \\
                                   &         &         &  (0.013)&         \\
True News                          &         &         &         &   -0.026\\
                                   &         &         &         &  (0.007)\\
Unskewed x True News               &         &         &         &   -0.026\\
                                   &         &         &         &  (0.013)\\
Question FE                        &      Yes&      Yes&       No&      Yes\\
Round FE                           &      Yes&      Yes&      Yes&      Yes\\
Subject FE                         &      Yes&      Yes&      Yes&      Yes\\
Neutral News                       &       No&       No&      Yes&       No\\
\hline
Observations                       &     7882&     7882&    10499&     7882\\
\(R^{2}\)                          &     0.25&     0.25&     0.21&     0.25\\
Mean                               &    0.574&    0.574&    0.575&    0.574\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}

